Self-Boosted Automated Program Repair

Program repair is an integral part of every software system's life-cycle but can be extremely challenging. To date, researchers have proposed various automated program repair (APR) techniques to reduce efforts of manual debugging. However, given a real-world buggy program, a typical APR technique usually generates a large number of patches, each of which needs to be validated against the original test suite which incurs extremely high computation costs. Although existing APR techniques have already leveraged various static and/or dynamic information to find the desired patches faster, they are still rather costly. In a recent work, researchers proposed unified debugging to leverage the patch execution information during APR to help boost fault localization; in this way,the application scope of APR techniques can be extended to all possible bugs, e.g., the patch execution information during APR can help with manual repair of the bugs that cannot be automatically fixed. Inspired by unified debugging, this work proposes SeAPR (Self-Boosted Automated Program Repair), the first technique to leverage the earlier patch execution information during APR to help boost automated repair itself on-the-fly. Our basic intuition is that patches similar to earlier high-quality/low-quality patches should be promoted/degraded to speed up the detection of the desired patches. This experimental study on 12 state-of-the-art APR systems demonstrates that, overall, SeAPR can substantially reduce the number of patch executions with negligible overhead. Our study also investigates the impact of various configurations on SeAPR. Lastly, our study demonstrates that SeAPR can even leverage the patch execution information from other APR tools from the same buggy program to further boost APR.

==> outdated/old.tex <==
\subsection{Evaluation Metrics}
Our primary metric is the change in position of the first candidate after patch reordering, shown in Formula \ref{formula:metric-displacement}.

\begin{formula} {\dis{} - Displacement}
        \Delta{}P = P_{prioritized} - P_{baseline}
        \label{formula:metric-displacement}
\end{formula}


While \dis{} is useful to get the change on individual subjects, we use the below formula, \disAvg{}, to analyze the average \dis{} across subjects.

\begin{formula}{\disAvg{} - Average Displacement}
        Avg_\Delta{}_{P} = \dfrac{\Delta{}P}{\#Subjects}
        \label{formula:metric-average}
\end{formula}

Additionally, we further calculate the number of subjects per tool with improved displacements, \disBetter{} ($\Delta{}$P $<$ 0) and worsened displacements, \disWorse{} ($\Delta{}$P $>$ 0) as supplementary metrics.


%----------%
Program repair is an integral part of every software system's lifecycle, but program repair, even automated, is extremely expensive and time consuming. Though finding genuine repairs is crucial, it is also important to design to find repair quickly and efficiently for scalable real-world repair. \prapr{} is a state-of-the-art repair tool and executes magnitudes faster than the next leading repair tool, \sam{but still wastes at least ~120 hours of time costs (over 90\% )}. Minimizing patch generation costs and patch validation costs are two common methods to quicken repair techniques, but prioritizing high-quality patch candidates to execute first is another method to speed up automated repair techniques. Recent works apply unified debugging, using patch validation results, to significantly enhance fault localization. This paper investigates on-the-fly patch prioritization and for quicker automated program repair. \sam{Our results show that...} \sam{contribution sentence 1. contribution sentence 2, contribution sentence 3, etc}


\Comment{
\input{paper-sections/definitions/def-match-matrix}


% \subsection{Patch Priority Implications}
% \label{section:implications}

Again, the validations of high-quality patches are more likely to produce genuine repairs. By high-quality we mean any patch that improves any system functionality. Any patch that is not a high-quality patch defaults to a low-quality patch. Optimizing the order patch validation is crucial for developing quicker techniques, especially for performance-heavy techniques where the fully repair search space is impractical to exhaustively explore or in time-sensitive environments. Following existing unified debugging works, validation information from patches sooner may ultimately allow high-quality patches to be prioritized sooner. Once a sufficiently high-quality patch has been found (e.g. a plausible or correct patch), all future patch candidates can be skipped to save potentially huge amounts of time and resources. For instance, a study show that the costs for validation are more than \sam{...} the costs of patch generation! \highlight{[add something about the large validation time costs compare to generation/synthesis.]} 

Information about each patch, can be collected even before validation occurs. An example of these collectable features is the modified elements(s) per patch. The intuition is that patches with features similar to known high-quality patches are likely to also be high-quality and should therefore be prioritized. Likewise, patches rather similar to known low-quality patches should be deprioritized as they are likely to produce low-quality patches.
}

\Comment{\begin{table}[bt]
    \centering
    \begin{tabular}{c|c}
            \tp{}(\mathp{})   & $\sum{}_{\mathbf{p}'}${|\{ \mathe{} | \mathe{} $\in$ \mathRow{\mathmm{}}{\mathp{}} $\cap$ \mathRow{\mathmm{}}{\mathp{}'} $\wedge$ \mathp{}' $\in$ \mathPh{} \}|} \\\hline
            \tn{}(\mathp{})   & $\sum{}_{\mathbf{p}'}${|\{ \mathe{} | \mathe{} $\in$ \mathRow{\mathmm{}}{\mathp{}} $\cap$ \mathRow{\mathmm{}}{\mathp{}'} $\wedge$ \mathp{}' $\in$ \mathPh{} \}|} \\\hline
            \fp{}(\mathp{})   & $\sum{}_{\mathbf{p}'}${|\{ \mathe{} | \mathe{} $\in$ \mathRow{\mathmm{}}{\mathp{}} $\cap$ \mathRow{\mathmm{}}{\mathp{}'} $\wedge$ \mathp{}' $\in$ \mathPh{} \}|} \\\hline
            \fn{}(\mathp{})   & $\sum{}_{\mathbf{p}'}${|\{ \mathe{} | \mathe{} $\in$ \mathRow{\mathmm{}}{\mathp{}} $\cap$ \mathRow{\mathmm{}}{\mathp{}'} $\wedge$ \mathp{}' $\in$ \mathPh{} \}|}
    \end{tabular}
    \caption{Patch similarity computation for patch \mathp{} \lingming{modify accordingly}}
    \label{tab:my_label}
\end{table}}


\Comment{At this point, we can evaluate the effectiveness of our technique, shown in Table \ref{figure:example-evaluation}.
Column \textit{Patch Quality} represents a patch's actual quality post-validation.
Columns \textit{\baselineOld{}}, \textit{\baselineNew{}}, and \textit{\dratio{}} represent our evaluation metrics as detailed in Formula \ref{formula:displacement-ratio}.}


\Comment{After completely processing all patch, we see that \textit{plausible \patchd{}}
validated 2 patches sooner compared to its original validation position yielding a \dratio{} of $\dfrac{4-2}{4} = 50\%$.
This earlier validation will yield performance gains in any scenario where the entire repair search space is not exhausted, e.g. if the tool halts after finding any plausible patch. Even this simple examples show the great potential our approach has to improve \apr{} performance. Next, we discuss the specifics of our approach and evaluation study.}

\Comment{\patcha{} $\cap{}$ \patchb{} contains 1 element; E$_{1}$ while \patcha{} $-$ \patchb{} contains 2 elements; E$_{2}$ and E$_{3}$. Thus B's entries for columns \textit{Match} and \textit{Differ} are 1 and 2 respectively. Since \patchVal{} is a low-quality patch, \tn{} increments by 1 and \fp{} increments by 2 resulting in the tuple $(0,2,1,0)$. Finally we compute the similarity score with the \tftuple{} and observe a similarity of $0.71$. This process repeats for all patches \patchUn{} $\in$ \mathP{} to compute their Match / Differ, \tftuple{}, and similarity. After one full iteration, \patchd{} has the highest similarity and is therefore chosen as \patchVal{} for the next iteration, shown in Table \ref{figure:example-i2}.}

\Comment{A simple example will demonstrate exactly how our technique works in practice. Again, our default candidate patch are \textit{plausible patches} and default similarity formula is \textit{Ochiai}. First, we collect static information about each patch, each patches' original position and modified elements. In this example we have four patches with static information described in Table \ref{figure:similarity-baseline}. From this table we see each patch modifies a variable number of program elements, E$_{1}$ - E$_{4}$. For instance, \patcha{} modifies E$_{1}$, E$_{2}$, and E$_{3}$ while \patchb{} modifies only E$_{1}$. Additionally, we see the initial validation order of the patches represented by column \textit{Position}. Since \patcha{} was originally validated first, we process \patcha{} as \patchVal{}. We now determine \patcha{}'s quality classification. Table \ref{figure:example-evaluation} shows the validation matrix for all patches. From this table, we see t$_{1}$ and t$_{2}$ originally fail on the unmodified project. \patcha{} does not improve upon any original system functionality and is therefore classified as a low-quality patch.}



%\begin{equation}
%\label{equation:tpnew}
%\begin{split}
%\text{\tp{}[\mathp{}]} = & $\sum{}_{\mathbf{p}'}${|\{ \mathe{} | \mathe{} $\in$ \mathRow{\mathmm{}}{\mathp{}} $\cap$ \mathRow{\mathmm{}}{\mathp{}'} $\wedge$ \mathp{}' $\in$ \mathPh{} \}|}~+ %\\
%& $\sum{}_{\mathbf{p}'}${|\{ \mathe{} | \mathe{} $\in$ \mathRow{\mathmp{}}{\mathp{}} $\cap$ \mathRow{\mathmp{}}{\mathp{}'} $\wedge$ \mathp{}' $\in$ \mathPh{} \}|}
%\end{split}
%\end{equation}

% The possible reason is that most of the patches generated by these tools can make all failed tests pass, producing similar sets of high/low-quality patches for both partial and full matrices.

==> paper-sections/02_background.tex <==
\section{Background}

% This section discusses patch prioritization in practice (Section \ref{section:patch-prioritization}), unified debugging (Section \ref{section:unified-debugging}), the implications of successful patch prioritization (Section \ref{section:implications}), and two simple motivating examples (Section \ref{section:example}).
\lingming{should have two subsections: (1) automated program repair, and (2) unified debugging. For program repair, we need to more systematically explain the overall apr process, e.g., including fault localization, patch generation, and patch validation; then, we talk about different categories of repair techniques (not just prapr and tbar), including heuristic-based, constraint-based, and template-based ones; then we claim patch validation is expensive to motivate our work. You can refer to section  2.2 of your issta'21 submission. }
Manual repair is the most accessible and employed repair strategy. Developers manually debug the code until the fault is localized, at which point patches are synthesized until a successful patch is found. Despite the common employment of this strategy, manual repair consumes large amounts of human, time, and monetary resources. \highlight{some statistic about rather large average temporal cost of manual repair}. Furthermore, manual repair is hopelessly unscalable for any nontrivial real-world system. \highlight{compare of how long it takes Google to compile system with infeasibility to automatically repair such similar system(s)}. Resulting from these challenges, researchers have recently extensively investigated \textbf{automated program repair} as an alternative to manual repair.

Automated repair employs automated repair tools / system to \textbf{automatically find faulty code} and/or \textbf{create and test patch candidates}. There exist a wide class of repair tools, but one class is significantly more prevalent than the rest, generate-and-validate repair tools.

% \subsubsection{Generate and validate}
Generate-and-validate tools, such as \prapr{}~\cite{Ghanbari2019PracticalMutation} and \tbar{}~\cite{Liu2019TBAR:Repair}, generates a set of patch candidates and consequently evaluate these candidates for against failing system tests to find genuine repairs. Most modern generate-and-validate repair tools \cite{Durieux2016DynaMoth:Repair, Ghanbari2019PracticalMutation, Koyuncu2020FixMiner:Repair, Liu2019AVATAR:Violations, Liu2019TBAR:Repair, Liu2019YouSystems, Martinez2018Ultra-largeAstor, Martinez2016ASTOR:Demo, Xiong2017PreciseRepair, Xuan2017Nopol:Programs, Yuan2018ARJA:Programming, Wen2018Context-awareRepair} identify a set of \textit{mutation points} within faulty systems. As these mutation points are established, program variants on the mutation point are created and validated one-by-one. Once all variants on a given mutation point are exhausted, the process continues to the next mutation point until the tool processes every mutation point.

The continued development of these tools dramatically save time, human, and monetary costs compared to manual repair. Unfortunately, the decrease in these costs is often insufficient to scale these techniques in huge real-world applications. The size and complexity of real-world systems can often offset the advantages imposed by automated repair and make only the quickest, nichest tools feasible practice. Even worse, tools with large search spaces (e.g. tools with the capability to fix several types of bugs) almost always wastes resources processing low-quality patches before likely high-quality patches. 

For example, \prapr{} is the current state-of-the-art for Java systems, repairing more systems than any previous repair tool up to 10X faster than the next leading tools on average \cite{Ghanbari2019PracticalMutation}. Despite \prapr{}'s impressive performance boost, only ~10\% of faulty projects are actually automatically repaired, wasting resources on the remaining 90\% of projects. On its evaluation dataset ( $\sim$139 hours of repair attempt) \sam{14 hours of execution lead to successful repairs while the remaining 125 hours are wasted otherwise}. Plainly, this is a huge obstacle in program repair; validating all patch candidates simply wastes significantly time and effort. While ongoing research is being conducted to expand the scope of \apr{} tools (i.e. letting tools repair more bugs), time spent \textbf{even on systems with successful patches} can intuitively be minimized by executing high-quality patches sooner \sam{and potentially stopping validation after some criteria has been met}.

Most generate-and-validate tools identify mutation points and create an initially prioritized list of mutation points. Despite this, we \textit{rarely see} any further reordering or refinement performed during the repair process. In fact, of the 17 tools we consider (further detailed in Section \ref{section:tools}) \sam{only three dynamically change the number of mutation points after validation initiates}. Given the thorough research into minimizing other performance overheads, we find it surprising that little research towards prioritizing high-quality repair patches sooner in the validation process exists, especially when exhaustively exploring a tool's search space is expensive and so often infeasible in practice. Thus there exists this need to make current \apr{} techniques faster and one relatively unexplored avenue is patch prioritization during the validation process.

% \subsection{Unified Debugging}
% \label{section:unified-debugging}

Recent \textit{unified debugging} works demonstrate patch validation information is quite useful for \textbf{\textit{manual repair}} \cite{Lou2020, Benton2020}. In these works, patches are divided up into categories dependent on the individual test validation results on the patch. The goal in these papers is to improve fault localization for manual repair or automated repair, with the idea that code elements associated with high priority categories are more likely to relate to actual faulty locations. These techniques have demonstrated increased fault localization accuracy, at the method-level and statement-level, boosting results up to \sam{$\sim$600\%} over spectrum-based fault localization. 

% \subsection{Technique lead-in}

As these works prove the utility of the information and technique towards manual repair, we believe using similar information can be applied in the context of \textbf{automated program repair}; instead of boosting fault localization, we aim to improve the performance of repair tools by prioritizing high-quality patches sooner in the validation process. This combination of static information and \sam{dynamic validation information} will yield more efficient patch validation orderings and ultimately save time otherwise wasted attempting low-quality patches. As generate and validate tools are most prevalent, both in academia and practice, we exclusively focus on recent generate-and-validate \apr{} tools for this paper. Thus, this paper investigates patch prioritization for boosting automated repair techniques on-the-fly using information generated during the validation process. To the best of our knowledge, \textbf{this is the first paper investigating on-the-fly patch prioritization for program repair tools}.

% Traditionally this is achieved in three ways. First, time costs \textbf{generating patches} are minimized. \highlight{add slightly more details} Second, time costs \textbf{validating patches} are minimized. \sam{[add slightly more details]}. Finally, high-quality patch candidates can be \textbf{prioritized} while low-quality candidates are demoted or even skipped for validation.

% The former two methods are extensive areas of ongoing research and generally involve optimizing performance costs associated with patch generation and validation. \sam{cite common papers here} The latter method is comparatively underresearched and aims to minimize the number of low-quality patch candidates validated before high-quality candidates. By executing high-quality patches sooner, repair techniques will either observe the correct fix sooner or be able to halt all future patch validations once a successful repair candidate is sufficiently unlikely to appear. Both of these scenarios allow \apr{} tools to stop validating future patches, potentially saving huge amounts of time in the repair process. Recent work shows patch validation information consistently improves improve fault localization in numerous ways, e.g. up to a 590\% improvement over commonly used spectrum-based fault localization \cite{Lou2020, Benton2020}. In light of these works, we believe patch validation information can likewise be used to facilitate patch prioritization.

==> paper-sections/definitions/def-cleanfix.tex <==
% \subsubsection{CleanFix}

\begin{theorem}
\textbf{CleanFix}: Patches improving faulty functionality \textbf{without} compromising correct functionality. Specifically, given the set of originally failing tests, \highlight{t$_{f}$} and the set of originally passing test, \highlight{t$_{p}$}, (1) any\highlight{t $\in$ t$_{f}$} passes and (2) no \highlight{t $\in$ t$_{p}$} fails.
\end{theorem}

==> paper-sections/definitions/def-match-matrix.tex <==
\begin{theorem}
    \textbf{Match matrix}: Matrix \mathmm{} defines all elements modified within a patch.
    \tftuple{} is a tuple of the form (\tp{}, \tn{}, \fp{}, \fn{})
    Each block describes which \tftuple{} value increments given comparison result C$_{R}$ and \patchVal{} quality \mathquality{}.\lingming{this one can be moved to approach as it is our definition (maybe just remove as we already have something similar in approach)}
    \label{definition-match}
\end{theorem}

\input{tables/sec03/example-match-matrix}

==> paper-sections/definitions/def-negfix.tex <==
% \subsubsection{NegFix}

\begin{theorem}
\textbf{NoneFix}: Patches compromising correct functionality without improving faulty functionality. Specifically, given the set of originally failing tests, \highlight{t$_{f}$} and the set of originally passing test, \highlight{t$_{p}$}, (1) no \highlight{t $\in$ t$_{f}$} passes, and (2) any \highlight{t $\in$ t$_{p}$} fails.
\end{theorem}

==> paper-sections/definitions/def-noisyfix.tex <==
% \subsubsection{NoisyFix}

\begin{theorem}
\textbf{NoisyFix}: Patches improving faulty functionality \textbf{but also} compromising correct functionality. Specifically, given the set of originally failing tests, \highlight{t$_{f}$} and the set of originally passing test, \highlight{t$_{p}$}, (1) any \highlight{t $\in$ t$_{f}$} passes, and (2) any \highlight{t $\in$ t$_{p}$} fails.
\end{theorem}


==> paper-sections/definitions/def-nonefix.tex <==
% \subsubsection{NoneFix}

\begin{theorem}
\textbf{NoneFix}: Patches which neither improve or degrade functionality. Specifically, given the set of originally failing tests, \highlight{t$_{f}$} and the set of originally passing test, \highlight{t$_{p}$}, (1) no \highlight{t $\in$ t$_{f}$} passes, and (2) no \highlight{t $\in$ t$_{p}$} fails.
\end{theorem}


==> tables/sec03/evaluation-example.tex <==
\begin{table}[htb]
    \scalebox{1.0}{
    \centering
    \begin{tabular}{|c|c||c|c||c|}
        \hline
        
        \rowcolor{tablegray} & \textbf{Patch Quality} & \textbf{\baselineOld{}} & \textbf{\baselineNew{}} & \textbf{\dratio} \\
        
        \hline
        \hline
        
        \patcha{} & Low & 1 & 1 & - \\ 
        \patchb{} & Low & 2 & 4 & -50\% \\
        \patchc{} & High & 3 & 3 & 0\% \\ \rowcolor{tablegray}
        \textbf{\patchd{}} & \textbf{Plausible} & \textbf{4} & \textbf{2} & \textbf{50\%} \\ 

        \hline

    \end{tabular}
    }
    \caption{Example Evaluation\lingming{this table can be removed as tables 4 and 5 (after addressing my comments) will be enough to convey the same info}}
    \label{figure:example-evaluation}
\end{table}
